Private Robust Estimation by Stabilizing Convex Relaxations

We give the first polynomial time and sample $(\epsilon, \delta)$-differentially private (DP) algorithm to estimate the mean, covariance and higher moments in the presence of a constant fraction of adversarial outliers. Our algorithm succeeds for families of distributions that satisfy two well-studied properties in prior works on robust estimation: certifiable subgaussianity of directional moments and certifiable hypercontractivity of degree 2 polynomials. Our recovery guarantees hold in the "right affine-invariant norms": Mahalanobis distance for mean, multiplicative spectral and relative Frobenius distance guarantees for covariance and injective norms for higher moments. Prior works obtained private robust algorithms for mean estimation of subgaussian distributions with bounded covariance. For covariance estimation, ours is the first efficient algorithm (even in the absence of outliers) that succeeds without any condition-number assumptions. Our algorithms arise from a new framework that provides a general blueprint for modifying convex relaxations for robust estimation to satisfy strong worst-case stability guarantees in the appropriate parameter norms whenever the algorithms produce witnesses of correctness in their run. We verify such guarantees for a modification of standard sum-of-squares (SoS) semidefinite programming relaxations for robust estimation. Our privacy guarantees are obtained by combining stability guarantees with a new "estimate dependent" noise injection mechanism in which noise scales with the eigenvalues of the estimated covariance. We believe this framework will be useful more generally in obtaining DP counterparts of robust estimators. Independently of our work, Ashtiani and Liaw [AL21] also obtained a polynomial time and sample private robust estimation algorithm for Gaussian distributions.

==> content/moment-est-backup.tex <==
%!TEX root = ../main.tex
\section{Differentially Private Robust Moment Estimation}
In this section, we describe a differentially private robust moment estimation algorithm. The following is the main result of this section:

\begin{theorem}[Differentially Private Robust Moment Estimation] \label{thm:diff-priv-robust-moment-estimation-section}
Fix $\epsilon,\delta,\eta>0, k \in \N$. There exists a randomized algorithm $\Alg$ that takes input $n \geq n_0 = ??$ points $Y \subseteq \bbQ^d$, runs in time $(Bn)^{O(k)}$ (where $B$ is the bit complexity of the entries of $Y$) and either outputs ``reject'' or estimates $\hat{\mu},\hat{\Sigma}$ in $\bbQ^d$ and $\bbQ^{d \times d}$ respectively with the following guarantees:
\begin{enumerate}
    \item \textbf{Privacy: } $\Alg$ is $(\epsilon,\delta)$-differentially private with respect to the input $Y$, viewed as a $d$-dimensional database of $n$ individuals. 
    \item \textbf{Utility: } Suppose there exists a good set $X \subseteq \bbQ^d$ (see~\cref{def:goodset}) such that $|Y \cap X| \geq (1-\eta)n$ with mean $\mu_*$ and covariance $\Sigma_*$. Then, with probability at least $0.99$ over the random choices of the algorithm, $\Alg$ outputs estimates $(\hat{\mu},\hat{\Sigma})$ in $\bbQ^d$ and $\bbQ^{d \times d}$ respectively satisfying the following guarantees:
    \[
    \forall u \in \R^d, \text{  } \iprod{\hat{\mu}-\mu_*,u} \leq O(\sqrt{Ck}) \eta^{1-1/2k} \sqrt{ u^{\top} \Sigma_*u}\mcom
    \]
    and,
    \[
     (1-O(Ck) \eta^{1-1/k}) \Sigma_* \preceq \hat{\Sigma} \preceq (1+O(Ck)\eta^{1-1/k})\Sigma_* \mper
    \]
    \end{enumerate}
\end{theorem}

\Pnote{say this in intro} Observe that the privacy guarantees of the algorithm are (necessarily) \emph{worst-case}. The utility guarantees, however, hold only under the assumption that $Y$ is an $\eta$-corruption of a good set $X$. 


\subsection{Algorithm} 

\paragraph{Witness Producing Version of Robust Moment Estimation Algorithm} 
We will use the following (non-private) version of the robust moment estimation algorithm of~\cite{KS17} that uses the same constraint system $\cA$ as in~\cite{KS17}. Our algorithm itself, however, makes one key change (we call our version ``witness producing'' for reasons that will soon become clear) to that of~\cite{KS17} in order to obtain a private robust moment estimation algorithm. Instead of outputting estimates of the moments of the unknown distribution, our algorithm  outputs a sequence of non-negative weights $p_1, p_2,\ldots, p_n$ forming a probability distribution on the input set of points $Y$. The estimates can then be obtained by taking moments of the finite set $Y$ with respect to the probability distribution on $Y$ defined by the weights $p_i$s. This simple change is crucial to our \emph{worst-case} analysis of the resulting algorithm (i.e. even when the distributional assumption that $Y$ is an $\eta$-corruption of some good set $X$ is not met) and obtaining our privacy guarantees. As we discuss in Section~\ref{??}, our blueprint for modifying convex optimization based robust estimation algorithms appears to broadly applicable beyond the specific setting of robust moment estimation. 



\begin{mdframed}[frametitle={$\cA$: Constraint System for $\eta$-Robust Moment Estimation}]
        \begin{enumerate}
            \item $w_i^2 = w_i$ for each $1 \leq i \leq n$,
            \item $\sum_{i = 1}^n w_i \geq (1-\eta)n$, 
            \item $w_i (x_i' - y_i) = 0$ for $1 \leq i \leq n$, 
            \item $\frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^k \leq (Ck)^{k/2} \Paren{\frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^2}^{k/2}$. 
        \end{enumerate}
        \label{box:constraints}
\end{mdframed} 

\begin{mdframed}
\avnote{Algorithm sometimes rejects, so I added this. Please check.}
      \begin{algorithm}[Linearized Robust Moment Estimation]
        \label{algo:robust-moment-estimation-witness-producing}\mbox{}
        \begin{description}
        \item[Given:]
        A set of points $Y = \{y_1, y_2, \ldots, y_n\} \subseteq \bbQ^d$, $\eta > 0$, a parameter $k \in \N$.
            %A sample $Y = \{y_1,y_2,\ldots,y_n\}$ with set of inliers $\cI$ generated from $\cN(0,\Sigma_\ast)$, error bound $\delta$, and upper bound $B$ with $\Sigma_\ast\preceq B\cdot I$.
        \item[Output:]
        Either ``reject'' or a sequence of non-negative weights $p_1, p_2, \ldots, p_n$ satisfying $p_i \leq \frac{1}{(1-\eta)n}$ for each $i$. 
        \item[Operation:]\mbox{}
         Find a pseudo-distribution $\tzeta$ of degree $O(k)$ satisfying the constraint system $\cA$ on input $Y$ with outlier-rate $\eta$. If such a pseudo-distribution does not exist, then return ``reject.'' Otherwise, output weights $p \in [0,1]^n$ defined by $p_i = \frac{\pE_{\tzeta}[w_i]}{\sum_{i = 1}^n \pE_{\tzeta}[w_i]}$ for each $i$.  % and minimizing $\Pot(\tzeta) = \Norm{\pE_{\tzeta}[w]}_2^2$.  
        \end{description}
      \end{algorithm}
\end{mdframed} 
\subsection{Analysis of Witness-Producing Robust Estimation Algorithm}
\begin{definition}[Good Set]\label{def:goodset} \avnote{Should we call this $(C,k)$-good?}
A set of points $X \subseteq \R^d$ is said to be \emph{good} if:
\[
\sststile{2k}{v} \Set{\frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^{2k} \leq (Ck)^{k} \Paren{\frac{1}{n} \sum_{i = 1}^n \iprod{x_i,v}^2}^{k}} \mper
\]
\end{definition}

\avnote{I made some changes to the following lemma. Please check if it looks correct now.}
\begin{lemma}[Guarantees for Witness-Producing Robust Moment Estimation Algorithm] \label{lem:witness-producing-robust-moment-estimation}
Given a subset of of $n$ points $Y \subseteq \bbQ^d$ whose entries have bit complexity $B$, Algorithm~\ref{algo:robust-moment-estimation-witness-producing} runs in time $(Bn)^{O(k)}$ and either (a.) outputs ``reject,'' or (b.) returns a sequence of weights $0 \leq p_1, p_2, \ldots, p_n$ satisfying $p_1 + p_2 + \cdots + p_n = 1$ \pasin{I think we have $p_1 + \cdots + p_n = 1$ in the following section?} \avnote{I agree that the sum should be 1. I believe there are some other normalization issues throughout the paper, which I've attempted to fix, e.g., in \cref{lem:close-to-subgaussian-is-subgaussian}}.

Moreover, if there exists a good set $X \subseteq \R^d$ with mean $\mu_*$, covariance $\Sigma_*$ such that $|Y \cap X| \geq (1-\eta)n$, then \cref{algo:robust-moment-estimation-witness-producing} never rejects, and the corresponding estimates $\hat{\mu} = \frac{1}{n} \sum_i p_i y_i$ and $\hat{\Sigma} = \frac{1}{n} \sum_{i = 1}^n p_i (y_i -\hat{\mu})(y_i - \hat{\mu})^{\top}$ \pasin{Missing $p_i$'s here?} satisfy the following guarantees:
\begin{enumerate}
   \item \textbf{Mean Estimation: } \[
    \forall u \in \R^d, \text{  } \iprod{\hat{\mu}-\mu_*,u} \leq O(\sqrt{Ck}) \eta^{1-1/2k} \sqrt{ u^{\top} \Sigma_*u}\mcom
    \]
    \item \textbf{Covariance Estimation: }\[
     (1-O(Ck) \eta^{1-1/k}) \Sigma_* \preceq \hat{\Sigma} \preceq (1+O(Ck)\eta^{1-1/k})\Sigma_* \mcom
    \]
    \item \textbf{Witness: } For $C' \leq 6C + O(\sqrt{\eta})$, 
    \[
   \sststile{}{} \Set{ \frac{1}{n} \sum_{i=1}^n p_i \iprod{y_i - \hat{\mu}}^{2k} \leq  (C'k)^k \Paren{\frac{1}{n} \sum_{i=1}^n p_i \iprod{y_i - \hat{\mu}}^{2}}^k }
    \]
\end{enumerate}
\end{lemma}



\subsection{Private Robust Moment Estimation} 
We now describe our privatized version of the (witness-producing) robust moment estimation algorithm above. Our algorithm is described below. 

\begin{mdframed}
      \begin{algorithm}[Private Robust Moment Estimation]
        \label{algo:private-robust-moment-estimation}\mbox{}
        \begin{description}
        \item[Given:]
        A set of points $Y = \{y_1, y_2, \ldots, y_n\} \subseteq \bbQ^d$, parameters $\eta, \epsilon,\delta > 0$, $k \in \N$.
            %A sample $Y = \{y_1,y_2,\ldots,y_n\}$ with set of inliers $\cI$ generated from $\cN(0,\Sigma_\ast)$, error bound $\delta$, and upper bound $B$ with $\Sigma_\ast\preceq B\cdot I$.
        \item[Output:]
        Estimates $\hat{\mu}$ and $\hat{\Sigma}$ for mean and covariances. 
        \item[Operation:]\mbox{}
        \begin{enumerate}
        \item  \textbf{Feasibility Check: } Let $\eta' = \Lap(2\eta,\frac{1}{\epsilon' n})$. If there is no pseudo-distribution that is $2^{-n^{O(k)}}$-approximately consistent with $\cA$ on input $Y$ with outlier-rate $\eta'$, reject and halt. 
          % \item \textbf{Witness Check: } Find a pseudo-distribution $\tilde{\zeta}$ of degree $2t$ minimizing $\Norm{\pE_{\tzeta}[w]}_2$ consistent with $\cA$ with input $Y$ and outlier parameter $\eta'$. Check if the witness returned satisfies the certifiable-subgaussian property. If no such pseudo-distribution exists or the witness-check fails, reject. 
         \item  \textbf{Stable Outlier-Rate Selection: }Sample an integer $\tau \in [0,\eta'n]$ where the probability of any $\tau$ is proportional to $\exp(\frac{\epsilon}{4}\score_Y(\tau))$ for $\score_Y(\tau) = \max_{\gamma} \Paren{\gamma - \frac{1}{4L} \stab_Y(\tau,\gamma) - |\gamma-L|}$. Here $\stab_Y(\tau,\gamma)$ is defined in Definition~\ref{def:stability} and $L = \frac{10}{\epsilon'} (\ln n + \ln (1/\delta'))$. 
          % \item Find a pseudo-distribution $\tilde{\zeta}_{stable}$ of degree $2t$ consistent with $\cA$ with input $Y$ and outlier parameter $\eta'$. If $\Norm{\pE_{\tzeta_{stable}}[w]}_2^2>\frac{1}{(1-\eta')n}$, reject and halt. 
          % \item If $\Norm{\pE_{\tzeta_{stable}}[w]}_2^2 \geq \Norm{\pE_{\tzeta}[w]}_2^2 - 100/n^2$, exit the up-search loop. Otherwise, set $\tzeta = \tzeta_{stable}$ and continue the Up-search Loop. 

      	  \item \textbf{Robust Estimation: }Compute a pseudo-distribution $\tzeta$ minimizing $\Norm{\pE_{\tzeta}[w]}_2^2$ and satisfying $\cA$ on input $Y$ with outlier-rate $\eta'+ \tau/n$.  
      	  \item \textbf{Witness Checking: }Let $\beta \sim \Lap(0,100/n^2)$. Check that the weight vector $p= \pE_{\tzeta}[w]$ induces a $(C+\beta)$-certifiably subgaussian distribution on $Y$. If not, reject immediately. Otherwise: 
          \item \textbf{Noise Sampling: }Let $z \sim \cN(0,\frac{10\epsilon^{-1} \ln n + 10 \ln {(1/\delta)}}{ n^{1-1/2k}})^d$ and $Z \sim \cN(0,\frac{10\epsilon^{-1} \ln n + 10 \ln {(1/\delta)}}{\epsilon n^{1-1/k}})^{{{d+1} \choose 2}}$ where we interpret $Z$ has a symmetric $d \times d$ matrix with independent lower-triangular entries. 
          \item  \textbf{Noise Injection: }Output $\hat{\mu} = \pE_{\tzeta}[\mu]+ \pE_{\tzeta}[\Sigma]^{-1/2} z$ and $\hat{\Sigma} = \pE_{\tzeta}[\Sigma] + \pE_{\tzeta}[\Sigma]^{1/2}Z\pE_{\tzeta}[\Sigma]^{1/2}$. 
        \end{enumerate}

        \end{description}
      \end{algorithm}
\end{mdframed} 



\subsection{Privacy Analysis}
Our analysis of the privacy of \Alg is based on a sequence of claims about each of the steps of \Alg that cumulatively establish the stability of the behavior of \Alg on adjacent inputs $Y,Y'$. We will rely on the following simple but key observation in our analysis. 

The following lemma is easy to verify using the definition of pseudo-distributions. 
\begin{lemma}[Adjacent Pseudo-distributions] \label{lem:adjacent-pseudo-distribution}
Let $\tzeta$ be a pseudo-distribution of degree $2k$ that satisfies all the constraints in \ref{box:constraints} on input $Y = \{y_1, y_2, \ldots, y_n\}$ with outlier-rate $\eta$. Let $Y' \subseteq \R^d$ be adjacent to $Y$. Define an \emph{adjacent pseudo-distribution} $\tzeta'$ (that ``zeroes out $w_i$'') defined by $\pE_{\tzeta'}[ w_S p(X',\cdots)] = \pE_{\tzeta}[w_S p(X',\cdots)]$ if $i \not \in S$ and $\pE_{\tzeta'}[ w_S p(X',\cdots)] = 0$ if $i \in S$ for every polynomial $p$ in $X'$ and other auxiliary indeterminates in $\cA$. Then, $\tzeta'$ is a pseudo-distribution of degree $2k$ that satisfies all the constraints in \ref{box:constraints} on both inputs $Y'$ and $Y$ with outlier parameter $\eta+1/n$. 
\end{lemma}

This allows us to conclude the following basic calculus of our potential function: \pasin{Potential function is not yet defined.}
\begin{lemma}[Basic Facts about $\Pot$] \label{lem:basic-props-of-pot}
Suppose that for some $Y \subseteq \R^d$ of size $n$, some $t \in \N$ and $\eta' \in [0,\eta_0/4]$, there is a pseudo-distribution of degree $2t$ consistent with $\cA$ on input $Y$. Then, for every $\eta\geq \eta'$, the following holds:
\begin{enumerate}
    \item \textbf{Monotonicity:} $\Pot_{\eta+1/n}(Y) \leq \Pot_{\eta}(Y)$. In particular, $\Pot$ is monotonically decreasing as its subscript increases.
    \item \textbf{Lower Bound: } $\Pot_{\eta}(Y) \geq (1-\eta)^2 n$. 
    \item \textbf{Upper Bound: } $\Pot_{\eta}(Y) \leq (1-\eta)n$.
\end{enumerate}
\end{lemma}
\begin{proof}
The first fact follows immediately from Lemma~\ref{lem:adjacent-pseudo-distribution}. For the second, observe that any pseudo-distribution $\tzeta$ of degree $2t$ consistent with $\cA$ on input $Y$ with outlier rate $\eta$ must satisfy $\sum_{i = 1}^n \pE_{\tzeta}[w_i] \geq (1-\eta)n$. Thus, by Cauchy-Schwarz inequality, $\sum_{i=1}^n \pE[w_i]^2 \geq (\sum_{i=1}^n \pE[w_i])^2/n = (1-\eta)^2 n$. This completes the proof. For the last part, observe that $\pE_{\tzeta}[w_i] \leq 1$ for every $i$. Thus, $\sum_{i = 1}^n \pE_{\tzeta}[w_i]^2 \leq \sum_{i = 1}^n \pE_{\tzeta}[w_i] = (1-\eta)n$. 
\end{proof}

The first step of \Alg checks whether the sum-of-squares relaxation for the robust moment estimation is feasible on $Y$. In order to ensure stability of behavior on adjacent $Y$ and $Y'$, we perform this check with a noisy copy of the outlier-rate $\eta'$. The following lemma analyzes the stability of this step. 

\begin{lemma}[Stability of Feasibility Check] \label{lem:feasibility-check}
Let $Y$ and $Y'$ be adjacent sets of $n$ points in $\R^d$. Then, with probability at least $1-\delta'$, 
\[
\Pr[ \text{ Step 1 of \Alg does not reject on } Y ] \leq e^{\epsilon'} \Pr[ \text{ Step 1 of \Alg does not reject on } Y' ]\mcom
\] 
and,
\[
\Pr[ \text{ Step 1 of \Alg rejects on } Y ] \leq e^{\epsilon'} \Pr[ \text{ Step 1 of \Alg rejects on } Y']\mcom
\] 
\end{lemma}

\begin{proof}
We observe the following simple property: let $\tzeta$ be a pseudo-distribution of degree $2k$ consistent with $\cA$ on input $Y$ with outlier-rate $\eta'$. Consider the adjacent pseudo-distribution from Lemma~\ref{lem:adjacent-pseudo-distribution} that zeroes out $w_i$. Then, observe that $\tzeta'$ satisfies all the constraints of $\cA$ on input $Y'$ with outlier-rate $\eta'+1/n$. 

Next, observe that with probability at least $1-\delta'$, the $\eta'$ constructed in Step 1 is contained in $[1.1 \eta, 2 \eta]$ (as long as $n \gg \log (1/\delta')/\epsilon')$. Let us condition on this property in the following. 

Thus, if the feasibility check (Step 1) on input $Y$ passes with outlier-rate $\eta'$ then it must also pass on $Y'$ with outlier-rate $\eta'+1/n$. By our choice of the distribution of $\eta'$ ($2\eta + Lap(0,1/\epsilon^2 n^2)$) the probability of any value $\eta'$  and $\eta'+1/n$ is within a multiplicative factor of $e^{\epsilon'}$. 

By a similar argument, if the feasibility check fails for $Y$ with outlier-rate $\eta'$, then, it must also fail for $Y'$ with outlier-rate $\eta'-1/n$. By an argument similar to above, the ratio of probabilities of seeing $\eta'$ and $\eta'-1/n$ is within $e^{\epsilon'}$. This completes the proof. 
\end{proof}

\paragraph{Analysis of Stable Outlier-Rate Selection} 
The goal of the second step of \Alg is to find an outlier-rate $\eta''$ such that the strongly convex potential function $\Pot(\tzeta)$ on the pseudo-distribution we will eventually compute (in Step 3) is close on adjacent input points $Y,Y'$. We will later use the strong convexity of the $\Pot$ and the closeness guarantee on $\Pot$ on $Y,Y'$ to infer that the weight vector $p(Y)$ and $p(Y')$ output by the algorithm themselves are close. 

Our key algorithmic trick to ensure the closeness of the strongly convex potential $\Pot$ is to find a ``stable interval'' $[\eta'+(\tau-\gamma_*(\tau))/n, \eta'+(\tau+\gamma_*(\tau))/n]$ of outlier-rates $\eta''$ such that strongly convex potential function at near-optimal solutions must vary slowly as $\eta''$ varies in the the interval. We find such an interval via a variant of specialized exponential mechanism. 

\begin{definition}[Potential for $Y$ at outlier-rate $\eta$]
For any $Y \subseteq \bbQ^d$, let $\Pot_{\eta}(Y) = \Norm{\pE_{\tzeta}[w]}_2^2$ where $\tzeta$ is a pseudo-distribution of degree $2k$ consistent with $\cA$ on input $Y$ with outlier-rate $\eta$ and minimizing $\Norm{\pE_{\tzeta}[w]}_2^2$. If no such pseudo-distribution exists, set $\Pot_{\eta}(Y) = \infty$. 
\end{definition}


\begin{definition}[Stability] \label{def:stability}
Fix $\eta \in [0,\eta_0/4]$, $t \in \N$. Suppose for some $Y \subseteq \R^d$ of size $n$, there is a pseudo-distribution $\tzeta$ consistent with the constraint system $\cA$ on input $Y$ with outlier-rate $\eta$. For any positive integers $\gamma < \tau$, we define the stability of the $2\gamma$ length interval centered at $\tau$ to be 
\[
\stab_Y(\tau,\gamma) = \Pot_{\eta + (\tau-\gamma)/n}(Y)- \Pot_{\eta + (\tau+\gamma)/n}(Y)\mper
\]
\pasin{Should $\gamma(\tau)$ be defined here? I don't think it's defined anywhere else?}
\end{definition}

Observe that if there is a pseudo-distribution consistent with $\cA$ on $Y$ with outlier-rate $\eta'$ then there is a pseudo-distribution consistent with $\cA$ on $Y$ with any outlier-rate $\geq \eta'$. Thus, stability above is well-defined. 

\begin{definition}[Score Function]
Fix $Y \subseteq \R^d$ of size $n$, $t \in \N$, and $\eta' \in [0,\eta_0/4]$. 
For a parameter $L$, we define the following score function for every integer $\tau\in [0,\eta' n]$:
\[
\score_Y(\tau) = \max_{\gamma \in \N} \Paren{ \gamma -  \frac{1}{20L} \stab_Y(\tau, \gamma) - \Abs{\gamma-L}}\mper
\]
\end{definition}

\begin{lemma} \label{lem:comparison-of-stability}
Fix $\eta' \in [0,\eta_0/4]$, $t \in \N$. Suppose for some $Y \subseteq \R^d$ of size $n$, there is a pseudo-distribution $\tzeta$ consistent with the constraint system $\cA$ on input $Y$ with outlier-rate $\eta'$. Let $Y'$ be any collection of $n$ points in $\R^d$ differing from $Y$ in at most one point. Then, for any $\tau, \gamma$, 
\[
\stab_{Y'}(\tau,\gamma-1) \leq \stab_{Y}(\tau,\gamma)\mper
\]
\end{lemma}

\begin{proof}
Using Lemma~\ref{lem:adjacent-pseudo-distribution} and noting that if $\tzeta'$ is adjacent to $\tzeta$ then $\Norm{\pE_{\tzeta}[w]}_2^2-1 \leq \Norm{\pE_{\tzeta}[w]}_2^2 \leq \Norm{\pE_{\tzeta}[w]}_2^2$, we have:
\[
 \Pot_{\eta'+(\tau-\gamma+1)/n}(Y') \leq \Pot_{\eta'+(\tau-\gamma)/n}(Y)
\]
and
\[
 \Pot_{\eta'+(\tau+\gamma)/n}(Y) \leq \Pot_{\eta'+(\tau+\gamma-1)/n}(Y').
\]
Combining the two equations yields
\begin{align*}
 \stab_{Y}(\tau,\gamma-1) &= \Pot_{\eta'+ (\tau-\gamma+1)/n}(Y')-\Pot_{\eta'+(\tau+\gamma-1)/n}(Y')\\
 &\leq \Pot_{\eta'+ (\tau-\gamma)/n}(Y)-\Pot_{\eta'+(\tau+\gamma)/n}(Y)\\
 &= \stab_{Y}(\tau,\gamma).
\end{align*}



\end{proof}

\begin{lemma}[Sensitivity of Score Function] \label{lem:sensitivity-score-function}
Let $Y,Y'$ be set of $n$ points in $\R^d$ differing at most in one point. Suppose for some $t \in \N$ and $\eta' \in [0,\eta_0/4]$, there are pseudo-distributions $\tzeta, \tzeta'$ consistent with $\cA$ with outlier-rate $\eta'$ on inputs $Y$ and $Y'$ respectively. Then, for every $\tau >0$,
\begin{equation}
 |\score_Y(\tau)-\score_{Y'}(\tau)| \leq 2. \label{eq:scoresensitivity}
\end{equation}
\end{lemma}
\begin{proof}
It suffices to prove that $\score_{Y'}(\tau) \geq \score_{Y}(\tau)-2$. A symmetric argument then proves that $\score_{Y}(\tau) \geq \score_{Y'}(\tau)-2$, which establishes \eqref{eq:scoresensitivity}.

Let $\gamma_* = \arg \max_{\gamma < \tau} \Paren{\gamma -  \frac{1}{4L} \stab_Y(\tau, \gamma) - \Abs{\gamma-L}}$. Then, $\score_{Y}(\tau) = \gamma_* - \frac{1}{4L} \stab_{Y}(\tau,\gamma_*) - |\gamma_*-L|$. From Lemma~\ref{lem:comparison-of-stability}, we know that $\stab_{Y'}(\tau,\gamma_*-1) \leq \stab_Y(\tau,\gamma_*)$. Thus, it follows that
\begin{align*}
 \score_{Y'}(\tau) &\geq (\gamma_* - 1) - \frac{1}{4L}\stab_{Y'}(\tau,\gamma_*-1) - |(\gamma_*-1) - L|\\
 &\geq (\gamma_* - 1) - \frac{1}{4L}\stab_Y(\tau,\gamma_*) - |\gamma_*-1 - L|\\
 &\geq \gamma_* - 1 - \frac{1}{4L}\stab_Y(\tau,\gamma_*) - |\gamma_*-L| - 1\\
 &= \score_Y(\tau) - 2,
\end{align*}
as desired.
\end{proof}

\begin{lemma}[Existence of a Good Stable Interval] \label{lem:existence-of-good-interval}
Suppose for some $t \in \N$ and $\eta' \in [0,\eta_0/4]$, there are pseudo-distributions $\tzeta$ consistent with $\cA$ with outlier-rate $\eta'$ on inputs $Y$. 
For every $L$, there is a $\tau \in [0,\eta']$ such that $\score_Y(\tau,\gamma) \geq L/2$. 
\end{lemma}

\begin{proof}
Let $J$ be the set of all integers $j$ in $[0,\eta_0 n/4]$ such that $\Pot_{\eta'+j/n}(Y)-\Pot_{\eta'+(j+1)/n}(Y)\geq 10L$.
Then, observe that $\Pot_{\eta'}(Y)-\Pot_{\eta'+\eta'}(Y) \leq (1-\eta')n - (1-2\eta')^2n = (3\eta' -4 \eta'^2)n \leq 3 \eta' n$. Thus, by Markov's inequality, $|J|/(\eta'n) \leq 3/10L$. Now, consider picking a random integer $j \in [0,\eta' n]$. Then, by a union bound with probability at least $1- 3/10 = 7/10$ over the choice of $\tau$, the length $[\tau-L/2, \tau+L/2]$ does not contain any $j \in J$. Thus, $\stab_{Y}(\tau,L/2) \leq 10L^2$. Thus, $\score_{Y}(\tau,L/2) \geq L - \beta_1 (10L^2) - |L-L| \geq L/2$. 

\end{proof}


\begin{lemma}[Utility of Score Function]
Suppose for some $t \in \N$ and $\eta' \in [0,\eta_0/4]$, there are pseudo-distributions $\tzeta$ consistent with $\cA$ with outlier-rate $\eta'$ on inputs $Y$. 
Fix $\epsilon',\delta'>0$. 
Consider the following probability distribution on $\tau \in [0,\eta' n]$: choose any $\tau \in [0,\eta' n]$ with probability proportional to $\exp(\epsilon'/4 \score_{Y}(\tau))$. Then, for any $L > \frac{10}{\epsilon'} (\log n + \log 1/\delta')$, with probability at least $1-\delta'$, the $\tau$ so chosen satisfies $\gamma_*(\tau) > L/100$ and $\stab_{Y}(\tau,\gamma_*) < 40 L^2$. 
\end{lemma}

\begin{proof}
From Lemma~\ref{lem:existence-of-good-interval}, we know that there is a $\tau$ of score $L/2$. Observe that for such an interval, $|\gamma_*-L| < L/2$ or $\gamma_* \geq L/2$ and $\frac{1}{20L} \stab_Y(\tau,\gamma_*) < L/2$ or $\stab_Y(\tau,\gamma_*)< 10L^2$. Let's call such an interval ``good''.

Let's call any $\tau$ with $\score_{Y}(\tau)<L/100$ to be ``low scoring''. Then, the probability of any low scoring $\tau$ is a factor $\exp(L \epsilon/10)$ smaller than the probability of any good $\tau$. Since there are $n$ total points, the total probability mass of low scoring $\tau$s is at most $n \exp(L \epsilon/10) < \delta$ if $L > \frac{10}{\epsilon} (\log n + \log 1/\delta)$. Thus, with probability at least $1-\delta$, the output of the distribution in the lemma is a $\tau$ with positive score. 

Next, observe that if $\score_{Y}(\tau) \geq L/100$, then, $\gamma_*(\tau) \geq \gamma_*(\tau) - |\gamma_*-L|\geq L/100$  as desired. Similarly, we can also derive that $\gamma_* < 199 L/100$. Thus, $\gamma_*(\tau) - \frac{1}{20L} \stab_{Y}(\tau,\gamma_*) \geq \score_Y(\tau) \geq L/100$ or $\stab_Y(\tau,\gamma_*) < 20L (L/100 + 199 L/100) < 40L^2$. 

\end{proof}

The following is the key consequence of our stable outlier-rate selection mechanism:

\begin{lemma}[Stability of Interval]
Let $Y,Y'$ be any adjacent sets of $n$ points. Let $\zeta_Y(\eta',\tau)$ be the probability that \Alg on input $Y$  generates the outlier-rate $\eta'$ and interval mid-point $\tau$ generated in Steps 1 and 2 respectively. Then, we have:
\[
\frac{\zeta_Y(\eta',\tau)}{\zeta_{Y'}(\eta'+1/n, \tau-1)} \leq e^{2\epsilon'}
\]
\end{lemma}
\begin{proof}
Let's suppose $\zeta_Y(\eta',\tau)$ is non-zero (as otherwise, the claim is trivial). Then, we know that $\zeta_Y(\eta',\tau) = \zeta_Y(\eta') \cdot \zeta_Y(\tau \mid \eta')$. From Lemma~\ref{lem:feasibility-check}, we know that $\zeta_{Y}(\eta')/\zeta_{Y'}(\eta'+1/n) \leq e^{\epsilon'}$. Next, from Lemma~\ref{lem:sensitivity-score-function}, we know that $\zeta_{Y}(\tau \mid \eta')/\zeta_{Y}(\tau-1 \mid \eta'+1) \leq e^{\epsilon'}$. \pasin{$\eta' + 1$ should be changed to $\eta' + 1/n$?} Combining the two bounds completes the proof. 
\end{proof}

\begin{lemma}[Potential Stability Under Good Coupling]
Let $Y,Y'$ be adjacent subsets of $\bbQ^d$. 
Suppose \Alg chooses $(\eta',\tau)$ in Steps 1 and 2 on input $Y$ and $(\eta'+1/n, \tau-1)$ in Steps 1 and 2 on input $Y'$ respectively. Suppose further that $\gamma_Y(\tau),\gamma_{Y'}(\tau-1) \geq 100$. \pasin{Where is this lower bound on $\gamma$ used in the proofs?} Then, 
\[
\Abs{\Pot_{(\eta'+\tau)/n}(Y) - \Pot_{(\eta'+\tau)/n}(Y')} \leq 40L^2 \mper
\]

\end{lemma}
\begin{proof}
It is enough to prove that $\Pot_{(\eta'+\tau)/n}(Y) - \Pot_{(\eta'+\tau)/n}(Y') \leq 40L^2$ as a symmetric argument proves the other direction and completes the proof. 

Let $\tzeta$ be the pseudo-distribution that minimizes $\Norm{\pE_{\tzeta}[w]}_2^2$ while satisying $\cA$ on $Y'$ with outlier-rate $\eta' + \tau/n$ (computed in Step 3 of the algorithm on input $Y'$). Suppose $Y$ and $Y'$ differ on $i$-th sample point. Let $\tzeta_{adj}$ be the adjacent pseudo-distribution obtained by zeroing out $w_i$. Then, from Lemma~\ref{lem:adjacent-pseudo-distribution}, we know that $\tzeta_{adj}$ is consistent with $\cA$ on input $Y$ with outlier-rate $\eta'+(\tau+1)/n$. Further, $\Norm{\pE_{\tzeta_{adj}}[w]}_2^2 \leq \Norm{\pE_{\tzeta}[w]}_2^2$. Thus, $\Pot_{\eta' + (\tau+1)/n}(Y) \leq \Pot_{\eta'+\tau/n}(Y')$. Further, $\Abs{\Pot_{\eta'+ \tau/n}(Y)-\Pot_{\eta+(\tau+1)/n}} \leq \Abs{\Pot_{\eta'+(\tau-\gamma\tau)/n} - \Pot_{\eta'-(\tau-\gamma)/n}(Y)} \leq 40L^2$. This completes the proof. 
\end{proof}


\paragraph{Parameter Closeness from Potential Stability}
\begin{lemma}[Parameter Closeness from Stability of Potential] \label{lem:param-closeness}
Let $\tzeta, \tzeta'$ be pseudo-distributions minimizing $\Norm{\pE_{\tzeta}[w]}_2^2$ while being consistent with $\cA$ on input $Y,Y'$ respectively with outlier-rate $\eta'+\tau/n$ for $\tau \leq n\eta$. Let $p_i(Y) = \frac{\pE_{\tzeta}[w_i]}{\sum_i \pE_{\tzeta}[w_i]}$ for each $i$ and $p_i(Y') = \frac{\pE_{\tzeta'}[w_i]}{\sum_i \pE_{\tzeta'}[w_i]}$. Let $\hat{\mu}_1 = \sum_i p_i(Y) y_i$ and $\hat{\mu}_2 = \sum_i p_i(Y') y_i'$. Similarly, let $\hat{\Sigma}_1 = \sum_i p_i(Y) (y_i-\hat{\mu}_1) (y_i-\hat{\mu}_1)^{\top}$ and $\hat{\Sigma}_2 = \sum_i p_i(Y') ((y_i'-\hat{\mu}_1)(y_i'-\hat{\mu}_2)^{\top}$.  

Suppose that $p_i(Y), p_i'(Y)$ induce $2k$-certifiably $C_1,C_2$-subgaussian distributions on $Y,Y'$ respectively. Suppose further that $\stab_{Y,\eta'}(\tau,\gamma), \stab_{Y',\eta'}(\tau,\gamma) \leq 40L^2$ for $\gamma \geq 100$ and $\Norm{\pE_{\tzeta}[w]}_2^2 - \Norm{\pE_{\tzeta}[w]}_2^2 \leq O(L^2)$. 

Then, 
\[
(1-O(L/\sqrt{n})) \hat{\Sigma}_1 \preceq \hat{\Sigma}_2 \preceq (1+O(L/\sqrt{n})) \hat{\Sigma}_1 \mcom
\]
and, for every $u \in \R^d$, 
\[
\iprod{\hat{\mu}_1-\hat{\mu}_2,u} \leq O(L/\sqrt{n}) \sqrt{u^{\top}\hat{\Sigma}_1 u} \mper
\]

\end{lemma}

\begin{proof}
Let $\tzeta_{adj}$ be the adjacent pseudo-distribution of degree $2k$ obtained by zeroing out $w_i$ where $i$ is the index of the point that $Y$ and $Y'$ differ on. Then, from Lemma~\ref{lem:adjacent-pseudo-distribution}, we know that $\tzeta_{adj}$ satisfies $\cA$ on input $Y'$ with outlier-rate $\eta'+\tau/n+1/n$. Further, $\Abs{\Norm{\pE_{\tzeta'}[w]}_2^2 - \Norm{\pE_{\tzeta_{adj}}[w]}_2^2} \leq \Abs{\Norm{\pE_{\tzeta'}[w]}_2^2 - \Norm{\pE_{\tzeta}[w]}_2^2}+1 \leq 41L^2$. Further, by stability of $100$-length interval around $\tau$ for $Y$ and $Y'$, we must also have $\Pot_{\eta'+(\tau+1)/n}(Y') \geq \Pot_{\eta'+\tau/n}(Y')-40L^2$. Let $\tzeta''$ be an optimal pseudo-distribution of degree $2k$ consistent with $\cA$ on input $Y'$ with outlier-rate $\eta'+(\tau+1)/n$. Then, we must have that $\Abs{\Norm{\pE_{\tzeta_{adj}}[w]}_2^2-\Norm{\pE_{\tzeta''}[w]}_2^2} \leq 81L^2$. 

Now, $\Norm{}_2^2$ is a convex function and pseudo-distributions of degree $2k$ satisfying $\cA$ form a closed convex set. Thus, by Proposition~\ref{prop:pythagorean-theorem-convex-set}, we must have that:
\[
\Norm{\pE_{\tzeta_{adj}}[w]-\pE_{\tzeta''}[w]}_2^2 \leq \Abs{\Norm{\pE_{\tzeta_{adj}}[w]}_2^2-\Norm{\pE_{\tzeta''}[w]}_2^2} \leq 81L^2\mper
\]

Further, given that $\tzeta'$ is consistent with $\cA$ on input $Y'$ with outlier-rate $\eta'+\tau/n$, it is also consistent with $\cA$ on input $Y'$ with outlier-rate $\eta'+(\tau+1)/n$. Thus by a similar argument as above, we can also conclude that: 
\[
\Norm{\pE_{\tzeta'}[w]-\pE_{\tzeta''}[w]}_2^2 \leq 81L^2\mper
\] 

By triangle inequality, thus, we must have:
\begin{equation} \label{eq:final-closeness-bound}
\Norm{\pE_{\tzeta_{adj}}[w] - \pE_{\tzeta'}[w]}_2^2 \leq 400L^2\mper
\end{equation}

Now, $\tzeta'$ induces weights $p_i'(Y)$ that induce a $2k$-certifiably $C_2$-subgaussian distribution on $Y'$. Thus, by Lemma~\ref{lem:close-to-subgaussian-is-subgaussian}, $\tzeta_{adj}$ induces weights $p_{adj}$ that induce a $2k$-certifiably $(C_2+O(1/\sqrt{n}))$-subgaussian distribution on $Y'$. Combining \eqref{eq:final-closeness-bound} with Fact~\ref{fact:param-closeness-from-tv-closeness} completes the proof. 


\end{proof}

\paragraph{Witness Checks} 
Let's now show that if witness check succeeds on $Y$ with parameter $C'$ then it must also succeed on $Y'$ with $C'+O(\sqrt{\eta'})$. 


\begin{lemma} \label{lem:witness-check-succeeds}
Let $0 \leq p_i(Y) \leq \frac{1}{(1-2\eta')}$ be a sequence of non-negative weights adding up to $n$ that induce a $2k$-certifiable $C'$-subgaussian distribution on $Y$. Let $p_i(Y')$ be a sequence of non-negative weights adding up to $n$ on $Y'$ adjacent to $Y$ such that $\Norm{p(Y)-p(Y')}_1 \leq 400L^2$. Then, $p_i(Y')$ induces a $2k$-certifiable $C'+O(\sqrt{\eta'})$-subgaussian distribution on $Y$. 
\end{lemma}

\paragraph{Noise Injection in Estimate-Dependent Norms} 


\begin{definition}[Hockey-stick Divergence]
Let $p(x),q(x)$ be probability density functions on $\R^d$. The Hockey-stick divergence between $p,q$ is defined as:
\[
\int_{x \in \R^d} \max\{0, p(x)-e^{\epsilon}q(x)\} dx\mper
\] 
\end{definition}

\begin{fact}[$(\epsilon,\delta)$-differential privacy from Hockey-stick Divergence Bounds]
A randomized algorithm $\cA$ that takes input a database $Y \subseteq \R^d$ is $(\epsilon,\delta)$-differentially private iff for any adjacent pair of databases $Y,Y' \subseteq \R^d$, $D_{e^{\epsilon}}(\cA(Y),\cA(Y')) \leq \delta$. 
\end{fact}

% \begin{fact}[Basic Matrix Fact 1] \label{lem:basic-matrix-fact}
% Let $\Sigma$ be a $d \times d$ positive semidefinite matrix. Then, 
% \[
% \Norm{\Sigma^{1/2}-I}_F \leq \Norm{\Sigma-I}_F \mper
% \]

% \end{fact}
% \begin{proof}
% Let $\lambda_1, \lambda_2, \ldots, \lambda_d$ be the eigenvalues of $\Sigma$. Then, $\lambda_i^{1/2}$ are the eigenvalues of $\Sigma^{1/2}$. Observe that $\Norm{\Sigma-I}_F^2 = \sum_{i =1}^d (1-\lambda_i)^2$ and for every $i$, $|1-\lambda_i| = |1-\lambda^{1/2}| (1+\lambda^{1/2})$ or $|1-\lambda^{1/2}| \leq |1-\lambda_i|/(1+\lambda_i^{1/2} \leq |1-\lambda_i|$. Thus, $\Norm{\Sigma^{1/2}-I}_F^2 = \sum_{i =1}^n (1-\lambda_i^{1/2})^2 \leq \sum_{i =1}^n (1-\lambda_i)^2 = \Norm{\Sigma-I}_F^2$ as required. 
% \end{proof}

% \begin{fact}[Contraction of Frobenius Norms]
% For every $A,B \in \R^{d \times d}$, $\Norm{AB}_F \leq \Norm{A}_2 \Norm{B}_F$. 
% \end{fact}

\begin{lemma}
For any $d \times d$ PSD matrix $\Sigma$ satisfying $\Norm{\Sigma-I}_F \leq \beta$, $\det(\Sigma^{\otimes 2})\in (1 \pm \sqrt{\beta/d})^{2d^2}$. 
\end{lemma}
\begin{proof}
Let $\lambda_1, \ldots, \lambda_d$ be the eigenvalues of $\Sigma$. Then, $\sum_{i=1}^d (\lambda_i-1)^2 \leq \beta^2$. Under this constraint, $\prod_{i=1}^d\lambda_i$ is maximized when $\lambda_i = (1+\sqrt{\beta/d})$ for all $i$ in which case it equals $(1+\sqrt{\beta/d})^d$. Thus, $\deg(\Sigma) \leq (1+\sqrt{\beta/d})^d$. Thus, $\det(\Sigma^{\otimes 2}) \leq (1+\sqrt{\beta/d})^{2d^2}$. By a similar argument, $\det(\Sigma^{\otimes 2}) \geq (1-\sqrt{\beta/d})^{2d^2}$.
\end{proof}

\begin{lemma}
Fix $\epsilon,\delta>0$. 
Let $\Sigma \preceq 0$ be such that $\Norm{\Sigma-I}_F \leq \beta$ for $\beta < O(d^{-3}/\log(1/\delta)$. Let $Z$ be a symmetric random matrix such that for each $i \leq j \in [d]$, $Z_{i,j} \sim \cN(0,1)$ and are jointly independent. Then,
\[
D_{e^{\epsilon}} (Z, \Sigma^{1/2}Z \Sigma^{1/2}) \leq \delta\mper
\]
\end{lemma}

\begin{proof} 
Let $A = \Sigma^{1/2}$. Let $R_1 = Z$ and $R_2 = A ZA$. Notice that the lemma follows if we can prove that the ratio of the PDFs of $R_1$ and $R_2$ is contained in $[e^{-\epsilon}, e^{\epsilon}]$ with probability at least $1-\delta$. 

Observe that $R_1,R_2$ have jointly Gaussian distribution in $d^2$ dimensions with mean $0$. The covariance of $R_1$ is $I_{d^2}$. For $R_2$, observe that $(i,j)$th entry of $AZA  = \sum_{k} a_i(k) \iprod{a_j,Z_k}$ where $a_i$ is the $i$-th row of the matrix $A$. Each such entry is mean $0$ and has variance $\E[ \sum_k a_i(k)^2 \iprod{a_j,Z_k}^2  = \Norm{a_i}_2^2 \Norm{a_j}_2^2$ by recalling that $Z_k$s are independent random standard Gaussian vectors. Further, observe that the correlation between $(i,j)$ and $(i',j')$ entry of $AZA^{\top}$ is given by $\E \sum_{k,k'} a_i(k) \iprod{a_j,Z_k} a_{i'} (k') \iprod{a_{j'}, Z_{k'}} = \E \sum_{k} a_i (k) a_{i'} (k') \iprod{a_j,Z_k} \iprod{a_{j'},Z_k} = \iprod{a_i,a_{i'}} \iprod{a_j,a_{j'}}$ where in the first equality we used that $\E \iprod{a_j, Z_k} \iprod{a_{j'}, Z_{k'}} = 0$ if $k \neq k'$. Or, equivalently, the covariance of $AZA^{\top} = (AA^{\top})^{\otimes 2} = \Sigma^{\otimes 2}=M$(say). 

Observe, in particular, that since $\Norm{\Sigma-I}_F \leq \beta$, $(1-\beta)I \preceq \Sigma \preceq (1+\beta)I$. Thus, $(1-\beta)^2I \preceq M \preceq (1+\beta)^2I$. Thus, $(1-\beta)I \preceq M^{-1} \preceq (1+3\beta)I$ for any $\beta <1/2$. 

We can now understand the ratio of PDFs of $R_1$ and $R_2$. For any $U \in \R^{d^2}$, the ratio of the PDFs of $R_1$ to that of $R_2$ is $e^{-\Norm{U}_F^2/2+\Norm{U^{\top}M^{-1}U}/2} \cdot \det(M)$. Observe that $(1+\sqrt{\beta/d})^{2d^2} < e^{2d^{1.5} \sqrt{\beta}}) < e^{\epsilon/2}$ if $\beta < 0.25 \epsilon^2 d^{-3}$. 


Then, notice that $\Norm{U^{\top}M^{-1}U}-\Norm{U}_2^2 \in [-\beta \Norm{U}_2^2, 3\beta \Norm{U}_2^2]$. Now, with probability at least $1-\delta$ over the draw of $U$ from either of $R_1$ or $R_2$, $\Norm{U}_2^2 \in [(1-3\beta)d^2/\log 1/\delta, (1+3\beta) d^2 \log 1/\delta]$. Thus, if $\beta < \epsilon/2 d^{-2} 1/\log (1/\delta)$, then, $\Norm{U^{\top}M^{-1}U}-\Norm{U}_2^2 \in [-\epsilon/2,\epsilon/2]$. 

Combining the above two calculations yields that whenever $\beta < 0.25 \epsilon^2 d^{-3}/\log (1/\delta)$, with probability at least $1-\delta$, the ratio of the PDFs of $R_1$ and $R_2$ is within a factor of $e^{\epsilon}$ of each other. The lemma now follows. 

% In order to calculate the covariance, let's observe that for any matrix $A$, $\tr(\Sigma_2^{1/2} Z \Sigma_2^{1/2}A) = \tr(Z \Sigma_2^{1/2}A \Sigma_2^{1/2})$. Thus, the ``variance in direction $A$'' is $\E_Z \tr(Z \Sigma_2^{1/2} A \Sigma_2^{1/2})^2 = \Norm{\Sigma_2^{1/2} A \Sigma_2^{1/2}}_F^2$. Let $M$ be the $d^2 \times d^2$ matrix such that for any matrix $A$, when seen as a $d^2$ dimensional vector $vec(A)$, it holds that $vec(A)^{\top}Mvec(A) = \Norm{\Sigma_2^{1/2}A\Sigma_2^{1/2}}_F^2$. Then, from the above calculation, $M$ is the covariance matrix of $R_2$. 








\end{proof}

% \begin{lemma}\label{lem:dprejectalg}
% Let $\cA$ be an algorithm that takes a database $Y \subseteq \R^d$ as input and outputs either ``reject'' or an estimate $\Theta$ in $\R^p$. Suppose the following two conditions hold:
% \begin{enumerate}
% \item For any adjacent databases $Y,Y'$, $\frac{\Pr[ \cA(Y) \text{ outputs reject }]}{\Pr [\cA(Y') \text{ outputs reject }]}$, $\frac{\Pr[ \cA(Y) \text{ does not output reject }]}{\Pr[ \cA(Y') \text{ does not output reject }]} \leq e^{\epsilon/2}$ with probability at least $1-\delta/2$ over the randomness of $\cA$. 
% \item For any measurable subset $S \subseteq \R^p$, $\Pr[ \cA(Y) \in S \mid \cA(Y) \text{ does not reject } ]/\Pr[ \cA(Y') \in S \mid \cA(Y) \text{ does not reject } ] \leq e^{\epsilon/2}$ with probability at least $1-\delta/2$ over the randomness of $\cA$. 
% \end{enumerate}
% Then, $\cA$ is $(\epsilon,\delta)$-differentially private. 
% \end{lemma}


% \begin{proof}
% Suppose $Y, Y' \subseteq \R^d$ are adjacent databases. Let $E_1$ be the event for the first condition in the lemma statement that occurs with probability $\geq 1 - \delta/2$. Let $E_2$ be the event corresponding to the second condition which also occurs with probability $\geq 1-\delta/2$. By the union bound we have that $E_1 \cap E_2$ occurs with probability $\geq 1-\delta$.

% Now, assume $E_1 \cap E_2$ holds. Suppose $S \subseteq \R^p \cup \{\mathrm{reject}\}$. Note that if $S$ does not contain ``reject,'' then
% \begin{align}
%  \frac{\Pr[\cA(Y) \in S]}{\Pr[\cA(Y') \in S]} &= \frac{\Pr[ \cA(Y) \text{ does not output reject }]}{\Pr[\cA(Y') \text{ does not output reject }]} \cdot \frac{\Pr[ \cA(Y) \in S \mid \cA(Y) \text{ does not reject } ]}{\Pr[ \cA(Y') \in S \mid \cA(Y) \text{ does not reject } ]} \nonumber\\
%  &\leq e^{\epsilon/2} \cdot e^{\epsilon/2} \nonumber\\
%  &= e^{\epsilon}, \label{eq:noreject}
% \end{align}
% by the conclusions of $E_1$ and $E_2$.

% On the other hand, suppose $S$ contains ``reject,'' i.e., $S = S' \cup \{\mathrm{reject}\}$. Then, note that
% \begin{align*}
%  \frac{\Pr[\cA(Y) \in S]}{\Pr[\cA(Y') \in S]} &= \frac{\Pr[\cA(Y) \text{ outputs reject }] + \Pr[\cA(Y) \in S']}{\Pr[\cA(Y') \text{ outputs reject }] + \Pr[\cA(Y') \in S']}\\
%  &\leq e^\eps,
% \end{align*}
% since $\frac{\Pr[\cA(Y) \text{ outputs reject }]}{\Pr[\cA(Y') \text{ outputs reject }]} \leq e^{\epsilon/2} \leq e^\epsilon$ and $\frac{\Pr[\cA(Y) \in S']}{\Pr[\cA(Y') \in S']} \leq e^\epsilon$, which follows from an argument similar to \eqref{eq:noreject}.

% Hence, for any neighboring datasets $Y,Y'\subseteq \R^d$, it follows that with probability $\geq 1-\delta$, $\frac{\Pr[\cA(Y) \in S]}{\Pr[\cA(Y') \in S]} \leq e^\epsilon$, which implies that $\cA$ is $(\epsilon,\delta)$-differentially private, as desired.


% \end{proof}




\paragraph{Putting Things Together} 

\begin{lemma}[Coupling of Parameters]
Consider a run of \Alg on input $Y$ with parameters $\eta',\tau,C'$ (in steps 1,2,4 respectively). Suppose further that none of the steps 1 or 4 reject and $\gamma(\tau)\geq 100$. Then, \Alg on $Y'$ with parameters $\eta'+1/n, \tau-1, C'+O(\sqrt{\eta'})$ (in steps 1,2,4 respectively) does not reject and produces parameters $\hat{\mu}(Y'),\hat{\Sigma}(Y')$ satisfying:
for every $u \in \R^d$, 
\[
\iprod{\hat{\mu}(Y)- \hat{\mu}(Y'),u} \leq O(L/\sqrt{n}) \sqrt{u^{\top} \hat{\Sigma}(Y) u}\mcom
\]
\[
(1-O(L/\sqrt{n}) \hat{\Sigma}_1 \preceq \hat{\Sigma}_2 \preceq (1+O(L/\sqrt{n})) \hat{\Sigma}_1\mper
\]
\end{lemma}
\begin{proof}
Immediate from Lemma~\ref{lem:param-closeness} combined with Lemma~\ref{lem:witness-check-succeeds}.
\end{proof}




\begin{lemma}[Privacy Guarantee]
Set $\epsilon' = \epsilon/10$ and $\delta' = \delta/10$. Then, \Alg is $(\epsilon,\delta)$-differentially private with respect to the input $Y$ viewed as a $d$-dimensional database of $n$ individuals.
\end{lemma}
\begin{proof}

\end{proof}










